H\"older Continuity of the Gradient of Solutions to Doubly Non-Linear Parabolic Equations

This paper is devoted to studying the local behavior of non-negative weak solutions to the doubly non-linear parabolic equation \begin{equation*} \partial_t u^q - \text{div}\big(|D u|^{p-2}D u\big) = 0 \end{equation*} in a space-time cylinder. H\"older estimates are established for the gradient of its weak solutions in the super-critical fast diffusion regime $0<p-1< q<\frac{N(p-1)}{(N-p)_+}$ where $N$ is the space dimension. Moreover, decay estimates are obtained for weak solutions and their gradient in the vicinity of possible extinction time. Two main components towards these regularity estimates are a time-insensitive Harnack inequality that is particular about this regime, and Schauder estimates for the parabolic $p$-Laplace equation.

==> index.tex <==
%-----------------------------------------------------------------------
% Beginning of index.tex
%-----------------------------------------------------------------------
%
%  AMS-LaTeX sample file for a monograph index, as used by AMS document
%  classes for book series.  This is a data file input by chapter.tex.
%  It was copied from a .ind file prepared for another purpose, and is
%  given here only for the purpose of showing the output format of an
%  index in this series.
%
% *** DO NOT CREATE YOUR INDEX FILE BY HAND, or use this as a model. ***
%  Put \index{...} entries in your source files.  Put \makeindex and
%  \printindex in your driver file, as shown in the template, to produce
%  a .idx file.  When the .idx file is processed by the makeindex
%  program, it will produce the .ind file with correct page numbers.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theindex}

\item Absorbing barrier, 4
\item Adjoint partial differential operator, 20
\item $A$-harmonic function, 16, 182
\item $A^*$-harmonic function, 182

\indexspace

\item Boundary condition, 20, 22
\subitem Dirichlet, 15
\subitem Neumann, 16
\item Boundary value problem
\subitem the first, 16
\subitem the second, 16
\subitem the third, 16
\item Bounded set, 19

\indexspace

\item Diffusion
\subitem coefficient, 1 
\subitem equation, 3, 23
\item Dirichlet
\subitem boundary condition, 15
\subitem boundary value problem, 16

\indexspace

\item Elliptic
\subitem boundary value problem, 14, 158
\subitem partial differential equation, 14
\subitem partial differential operator, 19

\indexspace

\item Fick's law, 1
\item Flux, 1
\item Formally adjoint partial differential operator, 20
\item Fundamental solution
\subitem conceptional explanation, 12
\subitem general definition, 23
\subitem temporally homogeneous case, 64, 112

\indexspace

\item Genuine solution, 196
\item Green function, 156
\item Green's formula, 21

\indexspace

\item Harnack theorems
\subitem first theorem, 185
\subitem inequality, 186
\subitem lemma, 186
\subitem second theorem, 187
\subitem third theorem, 187
\item Helmhotz decomposition, 214
\item Hilbert-Schmidt expansion theorem, 120

\indexspace

\item Initial-boundary value problem, 22
\item Initial condition, 22
\item Invariant measure (for the fundamental solution), 167

\indexspace

\item Maximum principle
\subitem for $A$-harmonic functions, 183
\subitem for parabolic differential equations, 65
\subitem strong, 83

\indexspace

\item Neumann
\subitem boundary condition, 16
\subitem boundary value problem, 16
\subitem function, 179

\indexspace

\item One-parameter semigroup, 113

\indexspace

\item Parabolic initial-boundary value problem, 22
\item Partial differential equation
\subitem of elliptic type, 14
\subitem of parabolic type, 22
\item Positive definite kernel, 121

\indexspace

\item Reflecting barrier, 4
\item Regular (set), 19
\item Removable isolated singularity, 191
\item Robin problem, 16

\indexspace

\item Semigroup property (of fundamental solution), 64, 113
\item Separation of variables, 131
\item Solenoidal (vector field), 209
\item Strong maximum principle, 83
\item Symmetry (of fundamental solution), 64, 112

\indexspace

\item Temporally homogeneous, 111

\indexspace

\item Vector field with potential, 209

\indexspace

\item Weak solution
\subitem of elliptic equations, 195
\subitem of parabolic equation, 196
\subitem associated with a boundary condition, 204

\end{theindex}

%-----------------------------------------------------------------------
% End of index.tex
%-----------------------------------------------------------------------


==> preface.tex <==
%-----------------------------------------------------------------------------
% Beginning of preface.tex
%-----------------------------------------------------------------------------
%
% AMS-LaTeX 1.2 sample file for a monograph, based on amsbook.cls.
% This is a data file input by chapter.tex.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{Preface}


The purpose of this paper is to prove the H\"older continuity of the gradient of a doubly nonlinear parabolic equation.

\aufm{Verena B\"ogelein\\ Frank Duzaar\\ Ugo Gianazza\\ Naian Liao\\
Christoph Scheven}

%-----------------------------------------------------------------------------
% End of preface.tex
%-----------------------------------------------------------------------------

